Supernova Remnant Candidates Discovered by the SARAO MeerKAT Galactic Plane Survey

Context. Sensitive radio continuum data could remove the difference between the number of known supernova remnants (SNRs) in the Galaxy compared to that expected, but due to confusion in the Galactic plane, faint SNRs can be challenging to distinguish from brighter HII regions and filamentary radio emission. Aims. We wish to exploit new SARAO MeerKAT 1.3 GHz Galactic Plane Survey (SMGPS) radio continuum data, which covers $251\deg \le l \le 358\deg$ and $2\deg \le l \le 61\deg$ at $|b|\le 1.5\deg$, to search for SNR candidates in the Milky Way disk. Methods. We also use MIR data from the Spitzer GLIMPSE, Spitzer MIPSGAL, and WISE surveys to help identify SNR candidates. The identified SNR candidate are sources of extended radio continuum emission that lack MIR counterparts, are not known as HII regions in the WISE Catalog of Galactic HII Regions, and are not known previously as SNRs Results. We locate 237 new Galactic SNR candidates in the SMGPS data. We also identify and confirm the expected radio morphology for 201 objects listed in the literature as being SNRs and 130 previously-identified SNR candidates. The known and candidate SNRs have similar spatial distributions and angular sizes. Conclusions. The SMGPS data allowed us to identify a large population of SNR candidates that can be confirmed as true SNRs using radio polarization measurements or by deriving radio spectral indices. If the 237 candidates are confirmed as true SNRs, it would approximately double the number of known Galactic SNRs in the survey area, alleviating much of the difference between the known and expected populations.

==> bad_candidates_number.tex <==
40


==> candidates_bad.tex <==
G331.8$-$0.0  &  0.000  &  0.000  &  2.7  \\ 
G339.6$-$0.6  &  -0.584  &  $-$0.584  &  5.0  \\ 
G350.7+0.6  &  -0.600  &  $-$0.600  &  70.0  \\ 
G353.0+0.8  &  -0.800  &  $-$0.800  &  80.0  \\ 
G358.3$-$0.7  &  -0.771  &  $-$0.771  &  37.0  \\ 
G005.106+0.332  &  0.332  &  0.332  &  4.5  \\ 
G005.989+0.019  &  0.019  &  0.019  &  5.9  \\ 
G6.4500$-$0.5583  &  -0.552  &  $-$0.552  &  3.1  \\ 
G8.8583$-$0.2583  &  -0.258  &  $-$0.258  &  2.0  \\ 
G013.549+0.352  &  0.352  &  0.352  &  4.0  \\ 
G013.626+0.299  &  0.299  &  0.299  &  3.5  \\ 
G013.658$-$0.241  &  -0.241  &  $-$0.241  &  4.2  \\ 
G016.126+0.690  &  0.690  &  0.690  &  27.0  \\ 
G18.53$-$0.86  &  -0.860  &  $-$0.860  &  8.6  \\ 
G18.9$-$1.2  &  -1.200  &  $-$1.200  &  64.0  \\ 
G19.13+0.90  &  0.900  &  0.900  &  12.0  \\ 
G021.492$-$0.010  &  -0.010  &  $-$0.010  &  3.5  \\ 
G21.8+0.2  &  0.200  &  0.200  &  58.0  \\ 
G022.177+0.314  &  0.314  &  0.314  &  11.1  \\ 
G022.951$-$0.311  &  -0.311  &  $-$0.311  &  2.4  \\ 
G24.0$-$0.3  &  -0.340  &  $-$0.340  &  48.0  \\ 
G024.193+0.284  &  0.284  &  0.284  &  2.1  \\ 
G26.13+0.13  &  0.130  &  0.130  &  11.3  \\ 
G27.39+0.24  &  0.240  &  0.240  &  2.4  \\ 
G28.21+0.02  &  0.020  &  0.020  &  2.5  \\ 
G028.524+0.268  &  0.268  &  0.268  &  3.1  \\ 
G028.877+0.241  &  0.241  &  0.241  &  1.3  \\ 
G28.88+0.41  &  0.410  &  0.410  &  8.9  \\ 
G28.92+0.26  &  0.260  &  0.260  &  3.2  \\ 
G030.362+0.623  &  0.623  &  0.623  &  7.4  \\ 
G030.508+0.574  &  0.574  &  0.574  &  6.0  \\ 
G32.73+0.15  &  -0.510  &  $-$0.510  &  12.0  \\ 
G34.93$-$0.24  &  -0.248  &  $-$0.248  &  7.1  \\ 
G035.129$-$0.343  &  -0.343  &  $-$0.343  &  1.8  \\ 
G35.3$-$0.0  &  0.000  &  0.000  &  24.0  \\ 
G037.337+0.422  &  0.422  &  0.422  &  3.3  \\ 
G037.506+0.777  &  0.777  &  0.777  &  1.3  \\ 
G039.203+0.811  &  0.811  &  0.811  &  1.6  \\ 
G39.56$-$0.32  &  -0.320  &  $-$0.320  &  8.5  \\ 
G043.070+0.558  &  0.558  &  0.558  &  2.1  \\ 


==> interesting_number.tex <==
286


==> known.tex <==
G266.2$-$01.2  &  266.211  &  $-$1.017  &  38.4  &  G22  \\ 
G267.0$-$01.0  &  266.967  &  $-$1.005  &  0.5  &  SNRCat  \\ 
G269.7+00.0  &  269.638  &  0.030  &  21.5  &  SNRCat  \\ 
G279.0+01.1  &  278.958  &  0.761  &  67.2  &  G22  \\ 
G284.0$-$01.8  &  284.079  &  $-$1.880  &  0.4  &  SNRCat  \\ 
G284.2$-$00.4  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G284.3$-$01.8  &  284.279  &  $-$1.826  &  17.3  &  G22  \\ 
G285.1$-$00.5  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G286.5$-$01.2  &  286.217  &  $-$1.104  &  23.2  &  G22  \\ 
G287.4+00.6  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G289.7$-$00.3  &  289.707  &  $-$0.295  &  9.5  &  G22  \\ 
G290.1$-$00.8  &  290.102  &  $-$0.754  &  9.6  &  G22  \\ 
G291.0+00.1  &  291.011  &  0.079  &  13.3  &  SNRCat  \\ 
G291.0$-$00.1  &  291.033  &  $-$0.099  &  7.5  &  G22  \\ 
G292.2$-$00.5  &  292.142  &  $-$0.532  &  9.9  &  G22  \\ 
G293.8+00.6  &  293.766  &  0.608  &  11.8  &  G22  \\ 
G294.1$-$00.0  &  294.125  &  $-$0.046  &  21.7  &  G22  \\ 
G296.1$-$00.5  &  295.929  &  $-$0.547  &  33.1  &  G22  \\ 
G296.6$-$00.4  &  296.608  &  $-$0.388  &  6.8  &  SNRCat  \\ 
G296.7$-$00.9  &  296.661  &  $-$0.922  &  7.6  &  G22  \\ 
G296.8$-$00.3  &  296.885  &  $-$0.350  &  10.3  &  G22  \\ 
G298.5$-$00.3  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G298.6$-$00.0  &  298.573  &  $-$0.063  &  6.2  &  G22  \\ 
G299.3$-$01.5  &  299.294  &  $-$1.521  &  18.5  &  SNRCat  \\ 
G299.6$-$00.5  &  299.593  &  $-$0.476  &  8.0  &  G22  \\ 
G301.4$-$01.0  &  301.432  &  $-$1.006  &  14.4  &  G22  \\ 
G302.3+00.7  &  302.282  &  0.717  &  9.7  &  G22  \\ 
G304.1$-$00.2  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G304.6+00.1  &  304.585  &  0.126  &  4.6  &  G22  \\ 
G306.3$-$00.9  &  306.309  &  $-$0.890  &  2.2  &  G22  \\ 
G308.1$-$00.7  &  308.122  &  $-$0.672  &  9.2  &  G22  \\ 
G308.4$-$01.4  &  308.477  &  $-$1.373  &  8.2  &  G22  \\ 
G308.8$-$00.1  &  308.860  &  $-$0.199  &  8.8  &  G22  \\ 
G309.2$-$00.6  &  309.172  &  $-$0.698  &  8.3  &  G22  \\ 
G309.8+00.0  &  309.779  &  0.006  &  13.6  &  G22  \\ 
G310.6$-$00.3  &  310.618  &  $-$0.283  &  4.7  &  G22  \\ 
G310.8$-$00.4  &  310.816  &  $-$0.475  &  5.8  &  G22  \\ 
G310.9$-$00.3  &  310.887  &  $-$0.262  &  8.4  &  SNRCat  \\ 
G311.5$-$00.3  &  311.524  &  $-$0.340  &  2.4  &  G22  \\ 
G312.4$-$00.4  &  312.452  &  $-$0.423  &  17.6  &  G22  \\ 
G313.3+00.1  &  313.319  &  0.130  &  3.0  &  SNRCat  \\ 
G313.6+00.3  &  313.594  &  0.318  &  7.4  &  SNRCat  \\ 
G315.4$-$00.3  &  315.469  &  $-$0.253  &  12.4  &  G22  \\ 
G315.9$-$00.0  &  315.895  &  $-$0.015  &  10.0  &  G22  \\ 
G316.3$-$00.0  &  316.272  &  $-$0.021  &  12.9  &  G22  \\ 
G317.3$-$00.2  &  317.296  &  $-$0.258  &  6.8  &  G22  \\ 
G318.2+00.1  &  318.148  &  0.161  &  28.3  &  G22  \\ 
G318.9+00.4  &  318.918  &  0.426  &  13.1  &  G22  \\ 
G319.9$-$00.7  &  319.901  &  $-$0.674  &  5.1  &  G22  \\ 
G320.4$-$01.2  &  320.382  &  $-$1.232  &  18.0  &  G22  \\ 
G321.9$-$00.3  &  321.913  &  $-$0.312  &  15.9  &  G22  \\ 
G321.9$-$01.1  &  321.929  &  $-$1.069  &  16.0  &  G22  \\ 
G322.1+00.0  &  322.105  &  0.023  &  3.7  &  G22  \\ 
G325.0$-$00.3  &  322.462  &  0.084  &  9.7  &  SNRCat  \\ 
G322.5$-$00.1  &  322.471  &  $-$0.101  &  8.0  &  G22  \\ 
G322.7+00.1  &  322.684  &  0.078  &  7.3  &  SNRCat  \\ 
G322.9$-$00.0  &  322.886  &  $-$0.002  &  7.0  &  SNRCat  \\ 
G323.5+00.1  &  323.481  &  0.072  &  6.9  &  G22  \\ 
G323.7$-$01.0  &  323.591  &  $-$1.134  &  15.3  &  G22  \\ 
G323.9+00.0  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G324.1+00.0  &  324.117  &  0.046  &  5.1  &  SNRCat  \\ 
G326.3$-$01.8  &  326.310  &  $-$1.714  &  18.5  &  G22  \\ 
G327.1$-$01.1  &  327.139  &  $-$1.075  &  10.5  &  G22  \\ 
G327.2$-$00.1  &  327.239  &  $-$0.129  &  2.9  &  G22  \\ 
G327.4+00.4  &  327.276  &  0.520  &  11.4  &  G22  \\ 
G327.4+01.0  &  327.385  &  1.002  &  7.4  &  G22  \\ 
G328.4+00.2  &  328.412  &  0.225  &  3.3  &  G22  \\ 
G329.7+00.4  &  329.722  &  0.374  &  20.2  &  G22  \\ 
G330.2+01.0  &  330.155  &  0.977  &  5.5  &  G22  \\ 
G330.7+00.1  &  330.718  &  0.116  &  7.4  &  SNRCat  \\ 
G331.5$-$00.6  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G332.0+00.2  &  331.989  &  0.173  &  5.9  &  G22  \\ 
G332.4+00.1  &  332.387  &  0.127  &  7.3  &  G22  \\ 
G332.4$-$00.4  &  332.423  &  $-$0.373  &  5.5  &  G22  \\ 
G332.5$-$00.3  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G333.9+00.0  &  333.863  &  $-$0.046  &  6.0  &  SNRCat  \\ 
G334.0$-$00.8  &  333.895  &  $-$0.850  &  10.1  &  SNRCat  \\ 
G335.2+00.1  &  335.182  &  0.109  &  11.0  &  G22  \\ 
G336.4+00.2  &  336.386  &  0.191  &  0.5  &  SNRCat  \\ 
G336.7$-$00.3  &  336.658  &  $-$0.300  &  2.7  &  SNRCat  \\ 
G336.7+00.5  &  336.740  &  0.540  &  6.8  &  G22  \\ 
G336.9$-$00.5  &  336.846  &  $-$0.550  &  8.5  &  SNRCat  \\ 
G337.0$-$00.1  &  336.945  &  $-$0.116  &  3.2  &  G22  \\ 
G337.0$-$00.1  &  336.981  &  $-$0.129  &  0.8  &  G22  \\ 
G337.2+00.1  &  337.184  &  0.065  &  1.5  &  G22  \\ 
G337.2$-$00.7  &  337.210  &  $-$0.724  &  3.1  &  G22  \\ 
G337.3+01.0  &  337.336  &  0.959  &  6.6  &  G22  \\ 
G337.5$-$00.1  &  337.528  &  $-$0.111  &  3.9  &  SNRCat  \\ 
G337.8$-$00.1  &  337.807  &  $-$0.094  &  3.6  &  G22  \\ 
G338.1+00.4  &  338.076  &  0.424  &  7.6  &  G22  \\ 
G338.3$-$00.0  &  338.327  &  $-$0.044  &  4.2  &  G22  \\ 
G338.5+00.1  &  338.535  &  0.101  &  3.6  &  G22  \\ 
G340.4+00.4  &  340.405  &  0.422  &  4.9  &  G22  \\ 
G340.6+00.3  &  340.586  &  0.346  &  2.9  &  G22  \\ 
G341.2+00.9  &  341.116  &  0.830  &  14.9  &  G22  \\ 
G341.9$-$00.3  &  341.846  &  $-$0.306  &  4.2  &  G22  \\ 
G342.0$-$00.2  &  341.956  &  $-$0.200  &  5.5  &  G22  \\ 
G342.1+00.9  &  342.107  &  0.888  &  5.5  &  G22  \\ 
G343.1$-$00.7  &  343.072  &  $-$0.668  &  12.0  &  G22  \\ 
G344.7$-$00.1  &  344.682  &  $-$0.184  &  5.1  &  G22  \\ 
G344.7+00.1  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G345.1$-$00.2  &  345.063  &  $-$0.204  &  3.5  &  SNRCat  \\ 
G345.2+00.2  &  345.155  &  0.244  &  6.6  &  SNRCat  \\ 
G345.7$-$00.2  &  345.734  &  $-$0.186  &  3.2  &  G22  \\ 
G346.2$-$01.0  &  346.190  &  $-$0.984  &  4.0  &  SNRCat  \\ 
G346.6$-$00.2  &  346.611  &  $-$0.218  &  4.9  &  G22  \\ 
G347.3$-$00.5  &  347.362  &  $-$0.582  &  28.8  &  G22  \\ 
G348.5+00.1  &  348.454  &  0.094  &  4.7  &  G22  \\ 
G348.5$-$00.0  &  348.547  &  $-$0.003  &  5.1  &  G22  \\ 
G348.7+00.3  &  348.646  &  0.399  &  5.4  &  G22  \\ 
G348.9+01.1  &  348.860  &  1.126  &  6.5  &  SNRCat  \\ 
G348.9$-$00.4  &  348.960  &  $-$0.455  &  20.5  &  SNRCat  \\ 
G349.2$-$00.1  &  349.149  &  $-$0.092  &  4.0  &  G22  \\ 
G349.7+00.2  &  349.728  &  0.172  &  1.4  &  G22  \\ 
G350.1$-$00.3  &  350.065  &  $-$0.325  &  2.7  &  G22  \\ 
G350.2$-$00.8  &  350.219  &  $-$0.842  &  0.6  &  SNRCat  \\ 
G350.2$-$00.8  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G351.2+00.1  &  351.263  &  0.164  &  4.8  &  G22  \\ 
G351.7+00.8  &  351.710  &  0.819  &  8.1  &  G22  \\ 
G351.9$-$00.9  &  351.926  &  $-$0.959  &  6.9  &  G22  \\ 
G352.7$-$00.1  &  352.744  &  $-$0.125  &  4.1  &  G22  \\ 
G353.6$-$00.7  &  353.541  &  $-$0.670  &  16.7  &  G22  \\ 
G354.1+00.3  &  354.055  &  0.281  &  6.4  &  SNRCat  \\ 
G354.1+00.1  &  354.166  &  0.053  &  4.5  &  G22  \\ 
G354.4+00.0  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G354.8$-$00.8  &  354.864  &  $-$0.764  &  10.3  &  G22  \\ 
G355.4+00.7  &  355.345  &  0.627  &  24.0  &  G22  \\ 
G355.6$-$00.0  &  355.675  &  $-$0.078  &  3.9  &  G22  \\ 
G356.3$-$00.3  &  356.312  &  $-$0.357  &  5.2  &  G22  \\ 
G356.3$-$01.5  &  356.322  &  $-$1.535  &  10.1  &  G22  \\ 
G357.7+00.3  &  357.706  &  0.324  &  13.8  &  G22  \\ 
G357.7$-$00.1  &  357.714  &  $-$0.112  &  9.7  &  G22  \\ 
G358.1+00.1  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G358.3+00.2  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G001.4$-$00.1  &  1.448  &  $-$0.148  &  5.6  &  G22  \\ 
G001.9+00.3  &  1.871  &  0.323  &  0.9  &  G22  \\ 
G003.7$-$00.2  &  3.779  &  $-$0.288  &  7.0  &  G22  \\ 
G003.8+00.3  &  3.860  &  0.393  &  10.9  &  G22  \\ 
G005.4$-$01.2  &  5.378  &  $-$1.222  &  18.6  &  G22  \\ 
G005.5+00.3  &  5.667  &  0.126  &  20.7  &  G22  \\ 
G005.7$-$00.1  &  5.699  &  $-$0.088  &  7.1  &  SNRCat  \\ 
G006.1+00.5  &  6.055  &  0.499  &  6.1  &  G22  \\ 
G006.1+01.2  &  6.183  &  1.107  &  8.0  &  G22  \\ 
G006.4$-$00.1  &  6.485  &  $-$0.102  &  19.0  &  G22  \\ 
G006.5$-$00.4  &  6.521  &  $-$0.483  &  10.6  &  G22  \\ 
G007.0$-$00.1  &  7.075  &  $-$0.102  &  9.1  &  G22  \\ 
G007.2+00.2  &  7.204  &  0.177  &  4.9  &  G22  \\ 
G008.3$-$00.0  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G008.9+00.4  &  8.778  &  0.477  &  18.9  &  G22  \\ 
G008.7$-$00.1  &  8.828  &  $-$0.153  &  18.9  &  G22  \\ 
G009.7$-$00.0  &  9.682  &  $-$0.077  &  5.0  &  G22  \\ 
G009.8+00.6  &  9.781  &  0.571  &  7.5  &  G22  \\ 
G009.9$-$00.8  &  9.974  &  $-$0.822  &  6.2  &  G22  \\ 
G010.5$-$00.0  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G011.0$-$00.0  &  11.037  &  $-$0.053  &  4.5  &  G22  \\ 
G011.1$-$00.7  &  11.130  &  $-$0.775  &  8.4  &  G22  \\ 
G011.1$-$01.0  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G011.2$-$00.3  &  11.180  &  $-$0.348  &  2.8  &  G22  \\ 
G011.1+00.1  &  11.186  &  0.128  &  5.1  &  G22  \\ 
G011.4$-$00.1  &  11.383  &  $-$0.073  &  4.8  &  G22  \\ 
G011.8$-$00.2  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G012.0$-$00.1  &  11.964  &  $-$0.097  &  3.4  &  G22  \\ 
G012.2+00.3  &  12.262  &  0.305  &  3.4  &  G22  \\ 
G012.5+00.2  &  12.580  &  0.217  &  2.7  &  G22  \\ 
G012.7$-$00.0  &  12.712  &  $-$0.008  &  3.2  &  G22  \\ 
G012.8$-$00.0  &  12.819  &  $-$0.023  &  1.5  &  G22  \\ 
G013.5+00.2  &  13.454  &  0.139  &  2.6  &  G22  \\ 
G014.1$-$00.1  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G014.1$-$00.1  &  14.209  &  $-$0.076  &  11.3  &  G22  \\ 
G014.3+00.1  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G015.4+00.1  &  15.427  &  0.161  &  7.3  &  G22  \\ 
G015.9+00.2  &  15.888  &  0.198  &  3.2  &  G22  \\ 
G016.0$-$00.5  &  16.053  &  $-$0.479  &  11.7  &  G22  \\ 
G016.4$-$00.5  &  16.419  &  $-$0.546  &  7.0  &  G22  \\ 
G016.7+00.1  &  16.735  &  0.082  &  2.6  &  G22  \\ 
G017.0$-$00.0  &  \nodata  &  \nodata  &  \nodata  &  G22  \\ 
G017.4$-$00.1  &  17.476  &  $-$0.117  &  5.0  &  G22  \\ 
G018.0$-$00.7  &  18.001  &  $-$0.691  &  0.3  &  SNRCat  \\ 
G018.1$-$00.1  &  18.150  &  $-$0.170  &  4.6  &  G22  \\ 
G018.5$-$00.4  &  \nodata  &  \nodata  &  \nodata  &  nan  \\ 
G018.6$-$00.2  &  18.620  &  $-$0.280  &  3.4  &  G22  \\ 
G018.8+00.3  &  18.770  &  0.390  &  10.3  &  G22  \\ 
G018.9$-$01.1  &  18.950  &  $-$1.077  &  19.0  &  G22  \\ 
G019.1+00.2  &  19.240  &  0.260  &  20.2  &  G22  \\ 
G020.0$-$00.2  &  19.990  &  $-$0.190  &  7.3  &  G22  \\ 
G020.4+00.1  &  20.460  &  0.150  &  5.4  &  SNRCat  \\ 
G021.0$-$00.4  &  21.030  &  $-$0.470  &  5.6  &  G22  \\ 
G021.5$-$00.9  &  21.500  &  $-$0.885  &  1.5  &  G22  \\ 
G021.6$-$00.8  &  21.640  &  $-$0.830  &  8.1  &  G22  \\ 
G021.8$-$00.6  &  21.830  &  $-$0.520  &  15.5  &  G22  \\ 
G021.9$-$00.1  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G022.7$-$00.2  &  22.710  &  $-$0.200  &  13.9  &  G22  \\ 
G023.3$-$00.3  &  23.270  &  $-$0.330  &  16.8  &  G22  \\ 
G024.7+00.6  &  24.550  &  0.630  &  15.2  &  G22  \\ 
G024.7$-$00.6  &  24.860  &  $-$0.660  &  13.1  &  G22  \\ 
G026.6$-$00.1  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G027.4+00.0  &  27.390  &  $-$0.010  &  3.1  &  G22  \\ 
G027.8+00.6  &  27.700  &  0.630  &  23.4  &  G22  \\ 
G028.6$-$00.1  &  28.610  &  $-$0.110  &  5.3  &  G22  \\ 
G029.4+00.1  &  29.369  &  0.101  &  5.3  &  SNRCat  \\ 
G029.6+00.1  &  29.564  &  0.110  &  3.1  &  G22  \\ 
G029.7$-$00.3  &  29.710  &  $-$0.237  &  2.4  &  G22  \\ 
G030.7+01.0  &  30.700  &  1.010  &  11.7  &  G22  \\ 
G031.5$-$00.6  &  31.544  &  $-$0.660  &  10.7  &  G22  \\ 
G031.9+00.0  &  31.870  &  0.017  &  4.1  &  G22  \\ 
G032.1$-$00.9  &  32.130  &  $-$0.960  &  21.5  &  G22  \\ 
G032.4+00.1  &  32.420  &  0.110  &  4.4  &  G22  \\ 
G032.6+00.5  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G032.8$-$00.1  &  32.790  &  $-$0.040  &  11.5  &  G22  \\ 
G033.2$-$00.6  &  33.180  &  $-$0.570  &  9.2  &  G22  \\ 
G033.6+00.1  &  33.670  &  0.030  &  6.7  &  G22  \\ 
G034.7$-$00.4  &  34.660  &  $-$0.400  &  19.2  &  G22  \\ 
G035.6$-$00.4  &  35.590  &  $-$0.440  &  8.6  &  G22  \\ 
G036.0+00.1  &  36.008  &  0.058  &  0.5  &  SNRCat  \\ 
G036.6$-$00.7  &  36.591  &  $-$0.818  &  6.5  &  G22  \\ 
G038.7$-$01.3  &  38.756  &  $-$1.151  &  25.1  &  G22  \\ 
G039.2$-$00.3  &  39.220  &  $-$0.320  &  4.5  &  G22  \\ 
G040.5$-$00.5  &  40.520  &  $-$0.510  &  12.5  &  G22  \\ 
G041.1$-$00.3  &  41.120  &  $-$0.314  &  2.7  &  G22  \\ 
G041.5+00.4  &  41.450  &  0.410  &  8.5  &  G22  \\ 
G042.0$-$00.1  &  41.960  &  $-$0.050  &  5.9  &  G22  \\ 
G042.8+00.6  &  42.773  &  0.666  &  13.4  &  G22  \\ 
G043.3$-$00.2  &  43.273  &  $-$0.182  &  3.1  &  G22  \\ 
G044.5$-$00.2  &  \nodata  &  \nodata  &  \nodata  &  SNRCat  \\ 
G045.7$-$00.4  &  45.610  &  $-$0.390  &  14.0  &  G22  \\ 
G046.8$-$00.3  &  46.767  &  $-$0.280  &  10.0  &  G22  \\ 
G049.2$-$00.7  &  49.185  &  $-$0.520  &  19.2  &  G22  \\ 
G053.4+00.0  &  53.416  &  0.042  &  4.2  &  G22  \\ 
G054.1+00.3  &  54.099  &  0.261  &  7.1  &  G22  \\ 
G054.4$-$00.3  &  54.500  &  $-$0.270  &  25.0  &  G22  \\ 
G055.0+00.3  &  54.935  &  $-$0.086  &  37.9  &  G22  \\ 
G057.2+00.8  &  57.240  &  0.820  &  6.7  &  G22  \\ 
G059.5+00.1  &  59.590  &  0.110  &  9.0  &  G22  \\ 


==> known_bad_number.tex <==
25


==> known_number.tex <==
215


==> old_number.tex <==
130

